Summarizing User-generated Textual Content: Motivation and Methods for Fairness in Algorithmic Summaries

As the amount of user-generated textual content grows rapidly, text summarization algorithms are increasingly being used to provide users a quick overview of the information content. Traditionally, summarization algorithms have been evaluated only based on how well they match human-written summaries (e.g. as measured by ROUGE scores). In this work, we propose to evaluate summarization algorithms from a completely new perspective that is important when the user-generated data to be summarized comes from different socially salient user groups, e.g. men or women, Caucasians or African-Americans, or different political groups (Republicans or Democrats). In such cases, we check whether the generated summaries fairly represent these different social groups. Specifically, considering that an extractive summarization algorithm selects a subset of the textual units (e.g. microblogs) in the original data for inclusion in the summary, we investigate whether this selection is fair or not. Our experiments over real-world microblog datasets show that existing summarization algorithms often represent the socially salient user-groups very differently compared to their distributions in the original data. More importantly, some groups are frequently under-represented in the generated summaries, and hence get far less exposure than what they would have obtained in the original data. To reduce such adverse impacts, we propose novel fairness-preserving summarization algorithms which produce high-quality summaries while ensuring fairness among various groups. To our knowledge, this is the first attempt to produce fair text summarization, and is likely to open up an interesting research direction.

==> methodology.tex <==

%\section{FairSumm: A Fairness-preserving Summarization Algorithm}
\section{Proposed Algorithm I for Fair Summarization}
\label{sec:fairsumm}

This section describes our first proposed algorithm for fair summarization. 
This algorithm, named {\tt FairSumm}, 
treats summarization as an optimization problem of a submodular, monotone objective function, where the fairness requirements are applied as constraints.
%Our proposed fairness-preserving summarization algorithm treats summarization as an optimization problem of a submodular, monotone objective function, where the fairness requirements are applied as constraints. In this section, we first establish the theoretical premise of our algorithm, and then describe our algorithm. 
The symbols used in this section are given in Table~\ref{tab:symbols}.



\subsection{Submodularity and Monotonicity}

%In this subsection, we will briefly some of important concepts underlying our proposed algorithm.

%\subsubsection*{Definitions}
\noindent \underline{\bf Definitions:}
Let $V = \{v_1, v_2, ..., v_n\}$ be the set of elements to be summarized, where each $v_i$ represents a textual unit (e.g., a tweet). 
We define a function $\mathcal{F}$ : $2^V$ $\rightarrow$ $\mathbb{R}$ (the set of real numbers)
%(where $\mathbb{R}$ is the set of real numbers) 
that assigns a real value to a subset (say, $S$) of $V$.
%, i.e. $S$ $\subseteq$ $V$. 
Our goal is to find $S$ ($\subseteq$ $V$) such that $|S| \le k$, where $k \in \mathbb{R}$ is the desired length of the summary (specified as an input), 
and for which $\mathcal{F}$ is maximized (i.e. $S$ = $argmax_{B\subseteq V} \mathcal{F}(B)$). 
So, from a set of textual units $V$, we look to find a summary $S$ that maximizes an objective function $\mathcal{F}$.

\vspace{2mm}
\noindent \textbf{Definition 1} (Discrete derivative)~\cite{Krause2014}: For $e$ $\in$ $V$ and a function  $f: 2^V \rightarrow \mathbb{R}$, let $\Delta(e|S)$ = $f(S \cup \{e\})$ -- $f(S)$ be the \textit{discrete derivative} of $f$ at $S$ with respect to $e$.

\vspace{2mm}
\noindent \textbf{Definition 2} (Submodularity): a function $f$ is \textit{submodular} if for every $A$ $\subseteq$ $B$ $\subseteq$ $V$ and $e$ $\in$ $V$ $\setminus$ $B$ (i.e. $e$ $\in$ $V$ and $e$ $\notin$ $B$), %the following holds
\begin{equation}
\Delta(e|A) \ge \Delta(e|B)
\end{equation}
This property is popularly called the {\it property of diminishing returns}.

\vspace{2mm}
\noindent \textbf{Definition 3} (Monotonicity): The function $f$ is \textit{monotone} (or \textit{monotone nondecreasing}) if for every $A$ $\subseteq$ $B$ $\subseteq$ $V$, $f(A)$ $\le$ $f(B)$


\begin{table} [tb]
\centering
%\small
\footnotesize
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{c|p{0.7\columnwidth}}
\hline
\textbf{Symbols} & \textbf{Meanings}\\
\hline
$V$ & Set of textual units to be summarized %(sentences in a document or tweets in a tweet collection) 
\\ \hline
$N$ & $|V|$, number of textual units to be summarized \\ \hline
$t$ & Number of classes to which the textual units in $V$ belong (e.g., $t=2$ for MeToo dataset, $t=3$ for USelection) \\ \hline
$Z_1, Z_2, \ldots, Z_t$ & The $t$ classes of the textual units \\ \hline
$S$ & Summary conforming to fairness notions ($S \subseteq V$) \\ \hline
$k$ & Desired length of summary, $|S|$ \\ \hline
$c_i$, $i = 1 \ldots t$ & Minimum number of textual units from class $Z_i$ to be included in $S$ (to satisfy a given fairness notion) \\ \hline

$\mathcal{F}$ & Objective function (overall goodness measure of $S$)\\ \hline
$\mathcal{L}$ & Coverage function 
(goodness measure of $S$)\\ \hline
$\mathcal{R}$ & Diversity reward function (goodness measure of $S$)\\ \hline
$sim(i,j)$ & Similarity score between two textual units $i, j \in V$ %and $j \in V$ 
\\ \hline
$\mathcal{M}$ & A (partition) matriod\\ \hline
$\mathcal{I}$ & Set of partitions of matriod $\mathcal{M}$\\ \hline
%$P$ & Number of partition matriods\\ \hline
$G$ & The optimized fair summary produced by Algorithm~\ref{algo:atga}\\
\hline
\end{tabular}
\caption{The main symbols used in Section~\ref{sec:fairsumm}.}
\vspace*{-10mm}
\label{tab:symbols}
\end{table}


\vspace{2mm}
%\subsubsection*{Properties} 
\noindent \underline{\bf Properties:}
We now discuss some of the important properties of monotone submodular functions which we will exploit in our problem formulation.

\vspace{2mm}
\noindent \textbf{Property 1} (The class of submodular functions is closed under non-negative linear combinations): Let $f_1$, $f_2$, ..., $f_n$ defined by \\$f_i$ : $2^V$ $\rightarrow$ $\mathbb{R}$ ($i$ = 1, 2, ..., $n$) be submodular functions and $\lambda_1$, $\lambda_2$, ..., $\lambda_n$ be non-negative real numbers. Then $\sum_{i=1}^{n} \lambda_i f_i$ is also submodular.\\
\textbf{Proof}: This is a well-known property of submodular functions (e.g., see \cite{Lin2011}),
hence the proof is omitted.
% \footnote{See \url{https://en.wikipedia.org/wiki/Submodular_set_function} as seen on 19th May, 2018.} 

\vspace{2mm}
\noindent \textbf{Property 2} (The class of monotone functions is closed under non-negative linear combinations): Let $f_1$, $f_2$, ..., $f_n$ defined by \\ $f_i$ : $2^V$ $\rightarrow$ $\mathbb{R}$ ($i$ = 1, 2, ..., $n$) be monotone functions and $\lambda_1$, $\lambda_2$, ..., $\lambda_n$ be non-negative real numbers. Then $\sum_{i=1}^{n} \lambda_i f_i$ is also monotone.\\
\textbf{Proof}: Let $A_1$ $\subseteq$ $A_2$ $\subseteq$ $V$. Then, since each $f_i$ is a monotone, $f_i(A_1)$ $\le$ $f_i(A_2)$. Let $F$ = $\sum_{i=1}^{n} \lambda_i f_i$.\\
\noindent \textit{Case I}: Let $\lambda_i$ $=$ 0, for all $i = 1, 2, \ldots, n$. 
Then, $F$ = 0 and is a constant (non-decreasing) function.\\
\textit{Case II}: Let $\lambda_i$ $>$ 0, for all $i = 1, 2, \ldots, n$. Then we can write
\begin{align*}
&A_1 \subseteq A_2
\Rightarrow f_i(A_1) \le f_i(A_2), \; \forall i \;\; \Rightarrow \sum_{i}^{n} f_i(A_1) \le \sum_{i}^{n}  f_i(A_2) \\
&\Rightarrow \sum_{i}^{n} \lambda_i f_i(A_1) \le \sum_{i}^{n} \lambda_i f_i(A_2) \;\;
[\because \; \lambda_i > 0, \forall i] \\
%[\mbox{since} \; \lambda_i > 0, \forall i] \\
&\Rightarrow F(A_1) \le F(A_2).
\end{align*}
\textit{Case III}: Let only some $m$ ($m$ $>$ 0 and $m$ $<$ $n$) $\lambda_i$s $>$ 0. Let, without any loss of generality,  such $\lambda_i$s be $\lambda_1$, $\lambda_2$, ..., $\lambda_m$. Then we have
\begin{align*}
&A_1 \subseteq A_2 
\Rightarrow f_i(A_1) \le f_i(A_2), \forall i \; \Rightarrow \sum_{i}^{m} f_i(A_1) \le \sum_{i}^{m}  f_i(A_2) \\
&\Rightarrow \sum_{i}^{m} \lambda_i f_i(A_1) \le \sum_{i}^{m} \lambda_i f_i(A_2) \hspace{1mm}%\\
[\because \lambda_i > 0, \mbox{for} \; i = 1, 2, \ldots, m)] \\
%[\mbox{since} \lambda_i > 0, \mbox{for} \; i = 1, 2, \ldots, m)] \\
&\Rightarrow \sum_{i}^{n} \lambda_i f_i(A_1) \le \sum_{i}^{n} \lambda_i f_i(A_2) \hspace{1mm} %\\
[\because \lambda_i = 0, \mbox{for} \; i = m+1, m+2, \ldots, n)] \\
%[\mbox{since} \lambda_i = 0, \mbox{for} \; i = m+1, m+2, \ldots, n)] \\
&\Rightarrow F(A_1) \le F(A_2)  
\end{align*}
This completes the proof.

\vspace{2mm}
\noindent \textbf{Property 3} (The class of monotone submodular functions is closed under non-negative linear combinations): Let $f_1$, $f_2$, ..., $f_n$ defined by $f_i$ : $2^V$ $\rightarrow$ $\mathbb{R}$ ($i$ = 1, 2, ..., $n$) be monotone submodular functions and $\lambda_1$, $\lambda_2$, ..., $\lambda_n$ be non-negative real numbers. Then $\sum_i \lambda_i f_i$ is also monotone submodular.\\
\textbf{Proof}: This follows trivially from Properties 1 and 2.

\vspace{2mm}
\noindent \textbf{Property 4}: Given functions $F$: $2^V$ $\rightarrow$ $\mathbb{R}$ and $f$: $\mathbb{R}$ $\rightarrow$ $\mathbb{R}$, the composition $F'$ = $f$ $\circ$ $F$ : $2^V$ $\rightarrow$ $\mathbb{R}$ (i.e., $F'(S)$ = $f(F(S))$) is nondecreasing sub-modular, if $f$ is non-decreasing concave and $F$ is nondecreasing submodular.\\ 
%~\cite{Lin2011}\\
%Sum of monotones is monotones, weighted sum of submodular is submodular
\textbf{Proof}: This is also a well-known property of submodular functions (e.g., see~\cite{Lin2011}), hence the proof is omitted.
% \footnote{See \url{https://en.wikipedia.org/wiki/Submodular_set_function} as seen on 19th May, 2018.} 

\vspace{-2mm}
\subsection{Formulation of the objective function for summarization}

We now look for an objective function for the task of extractive summarization. 
Following the formulation by 
Lin {\it et al.}~\cite{Lin2011}, we use monotone submodular functions to construct the objective function. We consider the following two aspects of an extractive text summarization algorithm:

\vspace{1mm}
\noindent \underline{\bf Coverage}: Coverage refers to amount of information covered in the summary $S$, measured by a function, say, $\mathcal{L}$. The generic form of $\mathcal{L}$ can be 
\begin{equation}
\mathcal{L}(S) = \sum_{i \in V, j \in S} sim_{i,j}
\label{eqn:coverage}
\end{equation}
where $sim_{i,j}$ denotes the similarity between two textual units (tweets, sentences, etc.) $i \in V$ and $j \in V$. 
Thus, $\mathcal{L}(S)$ measures the overall similarity of the textual units included in the summary $S$ with all the textual units in the input collection $V$.

%Note that, $\sum_{i \in V, j \in S} sim_{i,j}$ is monotone submodular. 
Note that $\mathcal{L}$ is monotone submodular.
$\mathcal{L}$ is monotonic since coverage increases by the addition of a new sentence in the summary. At the same time, $\mathcal{L}$ is submodular since the increase in $\mathcal{L}$ would be more when a sentence is added to a shorter summary, than when a sentence is added to a longer summary. 
There can be several forms of $\mathcal{L}$ depending on how $sim_{i,j}$ is measured, which we will discuss later in this paper.

\vspace{1mm}
\noindent \underline{\bf Diversity reward}: The purpose of this aspect is to avoid redundancy and reward diverse information in the summary. 
Let the associated function be denoted as $\mathcal{R}$. A generic formulation of $\mathcal{R}$ is 
\begin{equation}
\mathcal{R}(S) = \sum_{i=1}^K \sqrt{\sum_{j \in P_i \cap S} r_j}
\label{eqn:diversity}
\end{equation}
where $P_1, P_2, \ldots, P_K$ comprise a partition of $V$ such that $\large\cup_i P_i = V$ and $P_i \cap P_j$ = $\emptyset$ for all $i$ $\neq$ $j$; 
$r_j$ is a suitable monotone submodular function that estimates the importance of adding the textual unit $j$ to the summary.
The partitioning $P_1, P_2, \ldots, P_K$ can be achieved by clustering the set $V$ using any clustering algorithm (e.g., $K$-means), based on the similarity of items as measured by $sim(i,j)$.

$\mathcal{R}(S)$ rewards diversity since there is more benefit in selecting a textual unit from a partition (cluster) that does not yet have any of its elements included in the summary.
As soon as any one element from a cluster $P_i$ is included in the summary, the other elements in $P_i$ start having diminishing gains, due to the square root function.

The function $r_j$ is a `singleton reward function' since it estimates the reward of adding the singleton element $j \in V$ to the summary $S$. One possible way to define this function is:
\begin{equation}
r_j = \frac{1}{N} \sum_i sim(i,j)
\label{eqn:singleton-reward}
\end{equation}
which measures the average similarity of $j$ to the other textual units in $V$. 
Note that $\mathcal{R}(S)$ is monotone submodular by Property (4), since square root is a non-decreasing concave function. This formulation will remain monotone submodular if any other non-decreasing concave function is used instead of square root.

While constructing a summary, both coverage and diversity are important.
Only maximizing coverage may lead to lack of diversity in the resulting summary and vice versa. So, we define our objective function for summarization as follows:
\begin{equation}
\mathcal{F} = \lambda_1 \mathcal{L} + \lambda_2 \mathcal{R}
\label{eqn:summary-objective}
\end{equation}
where $\lambda_1$, $\lambda_1$ $\ge$ 0 are the weights given to coverage and diversity respectively. Note that, by Property (3), $\mathcal{F}$ is monotone submodular.
%We obtain L and R from equations (6) and (7) respectively (Section 5.1) of Lin et al.~\cite{Lin2011}. To compute $w_{i,j}$, apart from the formulation presented in this paper, we can use semantic similarity (e.g., cosine similarity between embedding vectors created from Word2Vec and GloVe). Finally, the {\it objective function} F is defined by equation (2) of this paper.

Our proposed fairness-preserving summarization algorithm will maximize $\mathcal{F}$ in keeping with some fairness constraints. We now discuss this step.
\vspace*{-4mm}
\subsection{Submodular Maximization using Partition Matroids} \label{sub:matroid}

For fairness-preserving summarization, we essentially need to optimize the submodular function $\mathcal{F}$ while ensuring that the summary includes at least a certain number of textual units from each class present in the input data.
%of the textual units (e.g., textual units written by male authors, and those written by female authors).
This problem can be formulated using the concept of partition matroids, as described below.

\vspace{2mm}
%\subsubsection*{Definitions}
\noindent \underline{\bf Definitions:} We start with some definitions that are necessary to formulate the constrained optimization problem.

\vspace{1mm}
\noindent \textbf{Definition 4} (Matroid): A matroid is a pair $\mathcal{M}$ = ($\mathcal{Z}$, $\mathcal{I}$), defined over a finite set $\mathcal{Z}$ (called the ground set)  and a family of sets $\mathcal{I}$ (called the independent sets), that satisfies the three properties:
\begin{enumerate}
\item $\emptyset$ (empty set) $\in$ $\mathcal{I}$.
\item If $Y$ $\in$ $\mathcal{I}$ and $X$ $\subseteq$ $Y$, then $X$ $\in$ $\mathcal{I}$.
\item If $X$ $\in$ $\mathcal{I}$, $Y$ $\in$ $\mathcal{I}$ and $|Y|$ $>$ $|X|$, then there exists $e$ $\in$ $Y$ $\setminus$ $X$ such that $X$ $\cup$ $\{e\}$ $\in$ $\mathcal{I}$.
\end{enumerate}

\vspace{1mm}
\noindent \textbf{Definition 5} (Partition Matroids): Partition matroids refer to a special type of matroids where the ground set $\mathcal{Z}$ is partitioned into disjoint subsets $\mathcal{Z}_1$, $\mathcal{Z}_2$, ..., $\mathcal{Z}_s$ for some $s$ and \\
$\mathcal{I}$ = \{$S$ | $S$ $\subseteq$ $\mathcal{Z}$ and $|S \cap \mathcal{Z}_i|$ $\le$ $c_i$, for all $i$ = 1, 2, ..., $s$\} 
for some given parameters $c_1$, $c_2$, ..., $c_s$.
Thus, $S$ is a subset of $Z$ that contains at least $c_i$ items from the partition $\mathcal{Z}_i$ (for all $i$), and $\mathcal{I}$ is the family of all such subsets.

\vspace{2mm}
%\subsubsection*{Formulation}
\noindent \underline{\bf Formulation of the constrained maximization problem:}
Consider that we have a set of control variables $z_j$ (e.g., gender, political leaning), each of which takes $t_j$ distinct values (e.g., male and female, democrat and republican). Each item in $\mathcal{Z}$ has a particular value for each $z_j$.

For each control variable $z_j$,  we can partition $\mathcal{Z}$ into $t_j$ disjoint subsets $\mathcal{Z}_{j1}$, $\mathcal{Z}_{j2}$, ..., $\mathcal{Z}_{jt_j}$, each corresponding to a particular value of this control variable. 
We now define a partition matriod $\mathcal{M}_j$ = ($\mathcal{Z}$, $\mathcal{I}_j$) such that
\begin{center}
$\mathcal{I}_j$ = \{$S$ | $S$ $\subseteq$ $\mathcal{Z}$ and $|S \cap Z_{ji}|$ $\le$ $c_j$, for all $i = 1, 2, \ldots, t_j$\}
\end{center}
for some given parameters $c_1$, $c_2$, ..., $c_{t_j}$.

Now, for a given submodular objective function $f$, a submodular optimization under the partition matriod constraints with $P$ control variables can be designed as follows:
\begin{equation}
\label{lab:eq}
Maximize_{S \subseteq \mathcal{Z}} \;\; f(S)
\end{equation}
\begin{center}
subject to $S \in \bigcap_{j=1}^P \mathcal{I}$.
\end{center}
A prior work by Du {\it et al.}~\cite{Du2013} has established that this submodular optimization problem under the matroid constraints can be solved efficiently with provable guarantees (see~\cite{Du2013} for details).


\subsection{Proposed summarization scheme}

In the context of the summarization problem, the ground set is $V$ (= $\mathcal{Z}$), the set of all textual units (sentences/tweets) which we look to summarize.
The control variables (stated in Section~\ref{sub:matroid}) are analogous to the sensitive attributes with respect to which fairness is to be ensured.
In this work, we consider only one sensitive attribute for a particular dataset (the gender of a user for the Claritin dataset, political leaning of a tweet for the USelection dataset, and the media source for the DUC06 dataset).
Let the corresponding control variable be $z$, and let $z$ take $t$ distinct values (e.g., $t = 2$ for the Claritin dataset, and $t=3$ for the USelection dataset).
Note that, as described in Section~\ref{sub:matroid}, the formulation can be extended to multiple sensitive attributes (control variables) as well.

Each textual unit in $V$ is associated with a class, i.e., a particular value of the control variable $z$ (e.g., is posted either my a male or a female). 
Let $Z_1$, $Z_2$, ..., $Z_t$ ($Z_i$ $\subseteq$ $V$, for all $i$) be the disjoint subsets of the textual units from the $t$ classes, each associated with a distinct value of $z$.
%Let $Z_1$ ($\subseteq$ $V$) be the set of all the sentences posted by males and $Z_2$ ($\subseteq$ $V$) be the set of all sentences posted by females. 
We now define a partition matroid $\mathcal{M}$ = ($V$, $\mathcal{I}$) in which $V$ is partitioned into disjoint subsets $Z_1$, $Z_2$, ..., $Z_n$ and
\begin{center}
$\mathcal{I}$ = \{$S$ | $S$ $\subseteq$ $V$ and $|S \cap Z_i|$ $\le$ $c_i$, $i$ = 1, 2, ..., $t$\}
\end{center}
for some given parameters $c_1$, $c_2$, ..., $c_t$.
In other words, $I$ will contain all the sets $S$ containing at most $c_i$ sentences from $Z_i$, $i$ = 1, 2, ..., $t$.

Outside the purview of the matroid constraints, we maintain the restriction that $c_i$'s are chosen such that\\
(1) $\sum_{i=1}^t c_i = k$ (the desired length of the summary $S$), and\\ 
(2) a desired fairness criterion is maintained in $S$. For instance, if equal representation of all classes in the summary is desired, then $c_i = \frac{k}{t}$ for all $i$. 

%the 80\% {\it adverse impact fairness criterion}~\cite{biddle-adverse-impact} is maintained in $S$.

\noindent We now express our fairness-constrained summarization problem as follows:
\begin{equation}
\label{lab:eq2}
Maximize_{S \subseteq V} \mathcal{F}(S)
\end{equation}
\begin{center}
subject to $S$ $\in$ $\mathcal{I}$.
\end{center}
where the objective function $\mathcal{F}(S)$ is as stated in Equation~\ref{eqn:summary-objective}.




\begin{algorithm}[tb]
 \caption{: FairSumm (for fair summarization)}
 \label{algo:atga}
 \begin{algorithmic}[1]

  \State Set $d$ = $max_{z \in V}$$\mathcal{F}(\{z\})$. 
  \State Set $w_t$ = $\frac{d}{(i+\delta)^t}$ for $t$ = 0, $\ldots$, $l$ where $l$ = $argmin_i$ [$w_i$ $\le$ $\frac{\delta d}{N}$], and $w_{l+1}$ = 0.
 % /* Here $N$ is the size of $V$, $\delta$ is chosen as 0.01 by Du et al.~\cite{Du2013} */
  \State Set $G$ = $\emptyset$
  \For{$t$ = 0, 1, $\ldots$, $l$, $l+1$}
  	\For{each $z \in $ and $G\cup \{z\}$ $\in$ $I$}
    	\If{$\mathcal{F}$($G\cup \{z\}$) - $\mathcal{F}$($G$) $\ge$ $w_t$}
        	\State Set $G$ $\leftarrow$ $G\cup \{z\}$
        \EndIf
    
    \EndFor

	
  \EndFor
  \State Output $G$
  
 \end{algorithmic}
\end{algorithm}



The suitable algorithm to solve this constrained submodular optimization problem, proposed by Du et al.~\cite{Du2013}, is presented as Algorithm~\ref{algo:atga}. The $G$ produced by Algorithm~\ref{algo:atga} is the solution of Equation~\ref{lab:eq2}. 
This algorithm is an efficient alternative to the greedy solution which has a time complexity of $\mathcal{O}(kN)$ where $N$ = $|V|$ and $k$ = $|S|$. On the other hand, it can be shown that the time complexity of Du et al.~\cite{Du2013} is $\mathcal{O}(min\{|G|N, \frac{N}{\delta}log\frac{N}{\delta}\})$, where $\delta$ is a factor (to be explained shortly). 
The reason for this efficiency is the fact that this algorithm does {\it not} perform exhaustive evaluation of all the possible submodular functions evolving in the intermediate steps of the algorithm. 
Instead, it keeps on decreasing the threshold $w_t$ by a dividing factor (1 + $\delta)$, which skips the evaluation of many submodular functions and sets the threshold to zero when it is small enough. 
It selects elements $z$ from the ground set (in our case, $V$) only at each threshold value to evaluate the marginal gain ($\mathcal{F}$($G\cup \{z\}$) - $\mathcal{F}$($G$)) without violating any constraints.


%The $G$ produced by Algorithm~\ref{algo:atga} is the solution of Equation~\ref{lab:eq2}. 
Note that, the theoretical guarantee of Algorithm~\ref{algo:atga} depends upon the number of partition matroids ($P$), i.e., the number of control variables, and the curvature ($c_f$) of $\mathcal{F}$ given by
\begin{center}
$c_f = max_{j \in V, \mathcal{F}(j)>0} \; \frac{\mathcal{F}(j) - \mathcal{F}(j|V \setminus \{j\})}{\mathcal{F}(j)}$
\end{center}
The approximation ratio is $\frac{1}{P+c_f}$ (see~\cite{Du2013} for details); in our setting, the number of partition matroids $P$ is $1$.


==> previous_other_methods.tex <==

\section{Alternative mechanisms for fair summarization} \label{sec:other_methods}

In this section, we discuss two alternative mechanisms for generating fair summaries. 
%We will compare the performances of these mechanisms with that of our proposed algorithm in the next section.

\subsection{Summarizing classes separately} \label{sub:classwise}

Suppose that the textual units in the input belong to $t$ classes $Z_1, Z_2, \ldots, Z_t$, and to conform to a desired fairness notion, the summary should have $c_i$ units from class $Z_i$, $i = 1, 2, \ldots, t$ 
%where $\sum_{i=1}^{t} c_i = k$ 
(using the same notations as in Section~\ref{sec:fairsumm}). 
The easiest way to generate a fair summary is to separately summarize the textual units belonging to each class $Z_i$, to produce a summary of length $c_i$, and finally to combine all the $t$ summaries to obtain the final summary of length $k$.
We refer to this method as the {\bf ClasswiseSumm} method -- specifically, we use our proposed algorithm, without any fairness constraints, to summarize each class separately. 

While this method is possibly the easiest to generate a fair summary, it is not clear how good the resultant summaries will be. We will evaluate this method in Section~\ref{sec:expts}.

%%%%%%%%%%%%%
\subsection{Fair ranking based summarization} \label{sub:fair-ranking}

Many summarization algorithms (including the unsupervised ones stated in Section~\ref{sec:background}) 
generate an importance score of each textual unit in the input.
The textual units are then ranked in decreasing order of this importance score, and the top-ranked $k$ units are selected to form the summary.
Hence, if the ranked list of the textual units can be made fair (according to some fairness notion), then selecting the top $k$ from this fair ranked list can be another way of generating fair summaries.

%Fairness in ranking systems is an important problem that has been addressed recently by Zehlike {\it et al.}~\cite{Zehlike2017}. 
%We discuss fairness in extractive text summarization in the light of the methodology developed in~\cite{Zehlike2017} since some summarization algorithms which produce summaries as a ranked list of textual units (sentences or tweets).
Zehlike {\it et al.}~\cite{Zehlike2017} recently proposed a fair-ranking scheme in  a {\bf two-class} setting, with a `majority class' and a `minority class' for which fairness has to be ensured adhering to a {\it ranked group fairness criterion} .
They proposed a ranking algorithm {\it FA*IR} that ensures that the proportion of the candidates/items from the minority class in a ranked list never falls below a certain specified threshold. 
Zehlike {\it et al.}~\cite{Zehlike2017} ensure two fairness criteria -- {\it selection utility} which means every selected item is more qualified than those not selected, and {\it ordering utility} which means for every pair of selected candidates, either the more qualified is ranked above or the difference in their qualifications is small. 





%To achieve this, Zehlike {\it et al.}~\cite{Zehlike2017} adhere to a {\it ranked group fairness criterion} which takes as input the minimum desired proportion ($p$) of the minority candidates/items in the ranked list.	
%However, this method is for {\it two classes} -- one, protected and the other, non-protected.

%Note that our problem of fair summarization is different from the problem setting of Zehlike et al.~\cite{Zehlike2017}. 
%Zehlike et al.~\cite{Zehlike2017}
%assume one of the classes to be a `minority class', and that fairness needs to be ensured only for the minority class (since there is no concern of under-representation of the majority class). 
%But in our setting, there is no pre-defined notion of minority and majority classes. 
%We have seen that the summary generated by various methods can be unfair towards any of the classes, including the class which has majority of textual units in the input data can be under-represented in the summary. 
%Hence,  we must ensure that the summary is fair towards each class. 
%For our summarization setting, we consider that class to be the majority class which has the higher number of textual units in the input data, while the class having lesser textual units in the input is considered the minority class.

%Zehlike {\it et al.}~\cite{Zehlike2017} also ensure two other fairness criteria -- {\it selection utility} which means every selected item is more qualified than those not selected, and {\it ordering utility} which means for every pair of selected candidates, either the more qualified is ranked above or the difference in their qualifications is small. 
%For our fair summarization problem, we aim at preserving {\it selection utility} in the summary, which means that the produced summary contains the most representative (important) textual units. However, ordering utility is not a strict requirement {\it within a summary} since (i)~goodness of a summary (e.g., as measured by ROUGE score) does not take order of textual units into account, and
%(ii)~once the textual units to be included in the summary are selected, it is customary to order them in the same order as they appear in the input document or the input stream, to ensure readability.


%%%%%%%%%%Commented by Abhisek on Aug 23, 2018%%%%%%%%%
\if{0}
\vspace{2mm}
\noindent \underline{{\bf Definitions:}} We state some definitions that are necessary to explain the methodology. The reader is referred to~\cite{Zehlike2017}for details.

\vspace{1mm}
\noindent \textit{Fair representation condition:} Let $F(x; n, p)$ be the cumulative distribution function for a binomial distribution $B$($n$, $p$).
Let $\mathcal{S}_{k,n}$ be the set of all permutations of size $k$ of the set $[n] = \{1, 2, ..., n\}$ of items to be ranked.
A set $\mathcal{s}$ $\subseteq$ $\mathcal{S}_{k,n}$  having $\mathcal{s}_p$ protected candidates fairly represents a protected class with minimum proportion $p$ at significance level $\alpha$ if $F(\mathcal{s}_p; k, p)$ $>$ $\alpha$.

\vspace{1mm}
\noindent \textit{Ranked group fairness condition:} A ranking $\mathcal{s}$ $\in$ $\mathcal{S}_{k,n}$ is said to satisfy this condition if for every prefix $\mathcal{s}|_{i}$ = $<$ $\mathcal{s}_{1}$, $\mathcal{s}_{2}$, ..., $\mathcal{s}_{i}$$>$, 1 $\le$ $i$ $\le$ $k$ and for $p$ and $\alpha$, if $\mathcal{s}|_{i}$ satisfies the \textit{fair representation condition} with proportion $p$ and significance $\alpha_c$ = c($\alpha$, $k$, $p$) which is corrected using~\cite{YangCorr2016}.
\fi
%%%%%%%%%%%%%%%%%Till Here%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{2mm}
\noindent \underline{{\bf Applying FA*IR algorithm for summarization:}} We use this algorithm for fair extractive text summarization as follows. We consider that class to be the majority class which has the higher number of textual units in the input data, while the class having lesser textual units in the input is considered the minority class.

\vspace{1mm}
\noindent \underline{Input:} The algorithm takes as input a set of textual units (to be summarized); the other input parameters ($k$, $q_i$, $g_i$ and $p$) are set as discussed below.

\vspace{1mm}
\noindent \underline{Parameter settings:} We set the parameters of FA*IR as follows.
\begin{compactitem}
\item \textit{Qualification ($q_i$) of a candidate:} In our summarization setting, this is the goodness value of a textual unit in the data to be summarized.
We set this value to the importance score computed by some standard summarization algorithm (e.g., the ones discussed in Section~\ref{sec:existing}) that ranks the text units by their importance scores.

\item \textit{Expected size ($k$) of the ranking:} The expected number of textual units in the summary ($k$).

\item \textit{Indicator variable ($g_i$) indicating if the candidate is protected:} 
%In our summarization setting, we do not have a pre-defined protected class. 
%However, to be consistent with the premise of {\it FA*IR} algorithm, 
We consider that class to be the minority class which has the lesser number of textual units in the input data. 

\item \textit{Minimum proportion ($p$) of protected candidates:} We will set this value in the open interval $]$0, 1$[$ (0 and 1 excluded) so that a particular notion of fairness is ensured in the summary. For instance, if we want equal representation of both classes in the summary, we will set $p = 0.5$.
\item \textit{Adjusted significance level ($\alpha_c$):} We regulate this parameter in the open interval $]$0, 1$[$. 
\end{compactitem}


\vspace{1mm}
\noindent \underline{Working of the algorithm:} Two priority queues $P_0$ (for the textual units from the majority class) and $P_1$ (for the textual units of the minority class), each with capacity $k$, are set to empty. 
Then $P_0$ and $P_1$ are initialized by the goodness values ($q_i$) of the majority and minority textual units respectively.
Then a ranked group fairness table is created which calculates the minimum number of minority items/candidates at each rank, given the parameter setting. 
If this table determines that a textual unit from the minority class needs to added to the summary (being generated), the algorithm adds the best element from $P_1$ to the summary $S$; otherwise it adds the overall best textual unit (from $P_0 \cup P_1$) to $S$. 
%Finally, the algorithm produces a fair summary $S$ of the input set $V$.

\vspace{1mm}
\noindent \underline{Output:} A fair summary ($S$) of desired length $k$, adhering to a particular notion of fairness.


\vspace{2mm}
\noindent 
Note that since the {\it FA*IR} algorithm provides fair ranking for two classes only~\cite{Zehlike2017}, we look to apply this algorithm for summarization of data containing textual units from exactly two classes. 
So, we report the summarization results using this methodology only on the Claritin dataset that has two classes -- Male and Female.
It is an interesting future work to design a fair ranking algorithm for more than two classes, and then to use the algorithm for summarizing data from more than two classes.









==> quality.tex <==
%Abhisek is adding observations in this file






\if{0}
\subsection{Few Tweets}
\red{By Male} \new{By Female}\\
\red {Let`s talk about absolute hypocrisy!  The left has stood by while these three have done their dirt!   Where's the outrage?!   Way to highjack \#MeToo movement for political gain. Sad!}\\
\red{It`s an excellent example of hypocrisy by Govt, when innocent men`s where roped in \#fakecases fake \#498a which lead them to \#suicide there wasn't anyone to come in support,  but when opportunistic like \#TanushreeDutta stepped in then committee was formed  \#MeToo4Publicity \#MeToo}\\
\red{\#MeToo4Publicity  The \#GenderBiasedLaws  were pushing men to commit suicide. \#MeToo is adding fuel to the fire ! \#Mangina  in firing line of \#FeministMafia.}\\
\red{When Settlement amount is the motive by falsely charging a man' it's called \#MeToo  Pls tk action on ppl filing \#FakeCases \& bring \#GenderNeutralLaws \#MeToo4publicity \#MensCommission.}\\
\red{Don't get fooled by \#MeToo gang . \#SpeakUpMan to Stop  \#MeToo4Publicity Don't get fooled by \#MeToo gang . \#SpeakUpMan to Stop abuse of Men and Demand Gender Neutral law. If Women do not do such crime , why they afraid for Gender neutral Law?}
\red{Pain knows no gender. When it hurts, it hurts equally, weather its a man or woman. Why there is discrimination on Gender. Every person deserves dignified treatment and happy life. \#MeToo  \#MeToo4Publicity  \#PurushAayog  \#PindadaanOfWives}\\
\red{If a woman shares a \#metoo without evidence, it`s taken to be true coz it`s a women`s testimony, a man coming out with \#HeToo story, people would be doubtful,  \& question the evidences, the intent \& will never except the man as victim. \#misandry must be understood. \#SpeakUpMan}\\
\red{Woman assaulted security guard \& put the blame on him. Policeman visited the lobby of the housing society. The women went out of control and stripped in front on policemen and security guard to run away from the situation. \#MeghaSharma \#HimToo \#MeToo}\\
\red{Instead of arresting this women @CPMumbaiPolice taking common man coz its \#MeToo \#MeTooIndia  \#MeToo4Publicity This is why \#Feminismiscancer  \#feminismismisandry \#Crimebywomen}\\
\new{ONLY 40 charges and thousands of cries for help. Too many are victim to \#UberRape and their voices aren`t being heard. \#TimesUp \#Metoo}\\
\new{If a woman is unveiled it gives a man the right 2 demand sexual favors.When it comes 2 sexual harassment in Islamic Republic it is always your fault if U dont wear hijab. Women using camera to expose sexual harassment. \#MyCameraIsMyWeapon is like  \#MeToo movement in Iran.}\\
\new{\#MeToo Pls empower the children in your houses to speak up. Let us discuss the evil in society if we want to tackle them! Increase collective awareness and reduce chances of fatalities. Better policies - At work, home, schools, Panchayat offices! \#TimesUp \#JusticeForRajalakshmi}\\
\new{Since my \#metoo moment:  * Someone tried to unsuccessfully shut down my Shopify stores. * Someone unsuccessfully reported my herbal business to Health Canada. *One abuser had a lawyer unsuccessfully send me a threatening cease \& desist letter. * Someone hacked my FB \& messages.}\\
\new{Breaking down gender stereotypes allows boys, girls, and all youth to be their best, most authentic selves. Join us and be a part of the change: \#GirlsToo \#MeToo}\\
\new{A long term solution would be the exact opposite of the two suggested here - gender sensitisation, not segregation so that the idea of exchange between different genders is normalised instead of being stigmatised further. \#MeToo \#Gender}\\
\new{Antifa is our new way of life. Move over you fascist white men. The patriarchy is over! \#resist \#MeToo \#TuesdayThoughts \#ImWithHer \#WomensMarch}\\
\new{Whatever happens to you in your life, you always have the choice to rise above your challenges. Choose NOT to be a victim. \#feminism \#metoo }\\
\fi{0}
